Traffic Control via Connected and Automated Vehicles: An Open-Road Field Experiment with 100 CAVs

The CIRCLES project aims to reduce instabilities in traffic flow, which are naturally occurring phenomena due to human driving behavior. These "phantom jams" or "stop-and-go waves,"are a significant source of wasted energy. Toward this goal, the CIRCLES project designed a control system referred to as the MegaController by the CIRCLES team, that could be deployed in real traffic. Our field experiment leveraged a heterogeneous fleet of 100 longitudinally-controlled vehicles as Lagrangian traffic actuators, each of which ran a controller with the architecture described in this paper. The MegaController is a hierarchical control architecture, which consists of two main layers. The upper layer is called Speed Planner, and is a centralized optimal control algorithm. It assigns speed targets to the vehicles, conveyed through the LTE cellular network. The lower layer is a control layer, running on each vehicle. It performs local actuation by overriding the stock adaptive cruise controller, using the stock on-board sensors. The Speed Planner ingests live data feeds provided by third parties, as well as data from our own control vehicles, and uses both to perform the speed assignment. The architecture of the speed planner allows for modular use of standard control techniques, such as optimal control, model predictive control, kernel methods and others, including Deep RL, model predictive control and explicit controllers. Depending on the vehicle architecture, all onboard sensing data can be accessed by the local controllers, or only some. Control inputs vary across different automakers, with inputs ranging from torque or acceleration requests for some cars, and electronic selection of ACC set points in others. The proposed architecture allows for the combination of all possible settings proposed above. Most configurations were tested throughout the ramp up to the MegaVandertest.

==> CompleteAuthorBios.tex <==
\begin{IEEEbiography}{Jonathan W.~Lee }{\,} (jonny5@berkeley.edu) received the B.S.~degree in engineering physics from the University of California, Berkeley and M.S.~and Ph.D.~degrees in mechanical engineering from Rice University. At Sandia National Laboratories (2011--13), he completed his postdoctoral appointment studying electrical and material properties via molecular dynamics simulations. He subsequently served as a senior data scientist and product manager on various teams at Uber Technologies, Inc.~(2014-2019). Since 2019, he has served as an engineering manager at the University of California, Berkeley and the program manager and Chief Engineer of CIRCLES.\end{IEEEbiography}  \begin{IEEEbiography}{Han Wang }{\,} (hanw@berkeley.edu) As of the submission of this thesis, Han is working on his Ph.D. in Transportation Engineering, as well as an M.S. degree in the Department of Electrical Engineering and Computer Sciences at U.C. Berkeley. His research focuses on the decentralized control of massive AV platforms and driving assistance utilizing computer vision techniques. \end{IEEEbiography}  \begin{IEEEbiography}{Kathy Jang }{\,} (kathyjang@berkeley.edu) is currently working on her Ph.D. in the Department of Electrical Engineering and Computer Sciences at U.C. Berkeley. Her research groups include Berkeley Artificial Intelligence Research (BAIR) and Berkeley Deep Drive (BDD).  Her focus is on robust reinforcement learning with applications to mixed-autonomy traffic.
\end{IEEEbiography}  \begin{IEEEbiography}{Amaury Hayat }{\,} (amaury.hayat@enpc.fr)
Amaury Hayat is a Professor of Mathematics at Ecole des Ponts Paristech since 2023. He is a Faculty member at the Research Center in Applied Mathematics of Ecole des Ponts Paristech since 2019. His research interests include control theory, partial differential equations, traffic control, and AI for mathematics.
 \end{IEEEbiography}  \begin{IEEEbiography}{Matthew Bunting }{\,} (matthew.r.bunting@vanderbilt.edu)  received a Ph.D. in Electrical and Computer Engineering at the University of Arizona, and is a research scientist in the Institute for Software Integrated Systems, at Vanderbilt University. His focus is on hardware development of autonomous vehicles, democratizing vehicle data collection and control through open source projects.
 \end{IEEEbiography}  \begin{IEEEbiography}{Arwa Alanqary }{\,} Arwa Alanqary received her B.S. in mechanical engineering from Alfaisal University in 2017 and M.S. degree in computational science and engineering from Massachusetts Instutte of Technology in 2019. She is currently a
 Ph.D. student in electrical engineering and computer sciences at the University of California, Berkeley. 
Her research interests include optimal control and optimization and learning in multi-agent systems.   
 \end{IEEEbiography}  \begin{IEEEbiography}{William Barbour }{\,} (william.w.barbour@vanderbilt.edu) 
is a Research Scientist (postdoctoral) at Vanderbilt University (Institute for Software Integrated Systems)
\end{IEEEbiography}  \begin{IEEEbiography}{Zhe Fu  }{\,} (zhefu@berkeley.edu) is a Ph.D. candidate in Transportation Engineering and a M.S. candidate at the Department of Electrical Engineering and Computer Sciences at U.C. Berkeley. Her research interests lie in traffic control and machine learning in mixed-autonomy traffic.\end{IEEEbiography}  \begin{IEEEbiography}{Xiaoqian Gong }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{George Gunter }{\,} is a PhD student in Civil and Environmental Engineering and the Institute for Software Integrated Systems. His research interests are on safety and security in applications of cyber-physical systems to civil infrastructure.\end{IEEEbiography}  \begin{IEEEbiography}{Sharon Hornstein }{\,} (sharon.hornstein@gm.com) is a researcher at the General Motors R\&D site in Israel. Sharon received her B.Sc., M.Sc. and Ph.D. degrees in Mechanical Engineering from the Technion, Israel. Her research interest is focused on the dynamic modeling of non-linear systems.   
 \end{IEEEbiography}  \begin{IEEEbiography}{Abdul Rahman Kreidieh }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Nathan Lichtlé }{\,} (nathanlct@berkeley.edu) is currently working on his Ph.D. in the Department of Electrical Engineering and Computer Sciences at U.C. Berkeley, and from the CERMICS group at École des Ponts ParisTech. His research groups include Berkeley Artificial Intelligence Research (BAIR) and Berkeley Deep Drive (BDD). His focus is on reinforcement learning and mixed-autonomy traffic.
 \end{IEEEbiography}  \begin{IEEEbiography}{Matthew W.~Nice }{\,} (matthew.nice@vanderbilt.edu)  received a M.Eng. in Cyber-Physical Systems, and is a doctoral candidate in the Department of Civil and Environmental Engineering, in the Institute for Software Integrated Systems, at Vanderbilt University. He has lead experimental research on the impact of technology in connected and automated vehicles on transportation systems. His research has been supported by multiple Dwight D. Eisenhower Transportation Fellowship Awards from FHWA.
 \end{IEEEbiography}  \begin{IEEEbiography}{William A.~Richardson }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Adit Shah }{\,} (aditshah@berkeley.edu) is an undergraduate student in the Department of Electrical Engineering and Computer Sciences at U.C. Berkeley. He focuses on machine learning and its societally beneficial applications.
 \end{IEEEbiography}  \begin{IEEEbiography}{Eugene Vinistky }{\,}  is currently an assistant professor in Civil Engineering at New York University. He completed his Ph.D. in the Department of Mechanical Engineering at U.C. Berkeley. His focus is on reinforcement learning and mixed-autonomy traffic.
 \end{IEEEbiography}  \begin{IEEEbiography}{Fangyu Wu }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Shengquan Xiang }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Sulaiman Almatrudi }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Fahd Althukair }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Rahul Bhadani }{\,} Rahul Bhadani is an assistant professor of Electrical \& Computer Engineering at The University of Alabama in Huntsville. He received his M.S (2017)., Ph.D. (2022) in Electrical \& Computer Engineering from the University of Arizona. He completed his postdoctoral appointment at Vanderbilt University, studying the modeling of microgrid components using SystemC-AMS. His research focuses on model-based system design for cyber-physical systems, and intelligent transportation. He has led the development of software tools to design, test and execute vehicle controllers for seminal experiments in transportation including the Arizona Ring-road experiment, and 100-car experiments on I-24 Nashville that demonstrated the impact of connected-and-automated vehicles in reducing urban traffic congestion and increasing fuel efficiency.  \end{IEEEbiography}  \begin{IEEEbiography}{Joy Carpio }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Raphaël Chekroun }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Eric Cheng }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Maria Teresa Chiri }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Fang-Chieh Chou }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Ryan Delorenzo }{\,} (rjd266@scarletmail.rutgers.edu) 
is a research assistant from Rutgers University - Camden.
 \end{IEEEbiography}  \begin{IEEEbiography}{Marsalis Gibson }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Derek Gloudemans }{\,} (derek.gloudemans@vanderbilt.edu) received a M.S. in Computer Science and is a doctoral candidate in the Department of Computer Science, in the Institute for Software Integrated Systems, at Vanderbilt University. He has led computer vision research and software implementation on the I-24 MOTION project. \end{IEEEbiography}  \begin{IEEEbiography}{Anish Gollakota }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Junyi Ji  }{\,} is  PhD student in Civil and Environmental Engineering and the Institute for Software Integrated Systems. His research interests are in the area of data-driven traffic flow theory and control. \end{IEEEbiography}  \begin{IEEEbiography}{Alexander Keimer }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Nour Khoudari }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Malaika Mahmood }{\,} (mm2878@scarletmail.rutgers.edu) 
is a research assistant from Rutgers University - Camden.
\end{IEEEbiography}  \begin{IEEEbiography}{Mikail Mahmood }{\,} (mm3194@camden.rutgers.edu) 
is a research assistant from Rutgers University - Camden.
 \end{IEEEbiography}  \begin{IEEEbiography}{Hossein Nick Zinat Matin }{\,} (h-matin@berkeley.edu) Hossein is a postdoctoral researcher at the University of California Berkeley. His research interest is partial differential equations and their applications in the theory of traffic flow. \end{IEEEbiography}  \begin{IEEEbiography}{Sean Mcquade }{\,} (sean.mcquade@rutgers.edu) 
Sean McQuade received a B.S.~degree in Mathematics from Virginia Polytechnic Institute and State University. He received a Ph.D.~degree in Computational and Integrative Biology from Rutgers–Camden. He currently works as a Postdoc at Rutgers–Camden as a senior researcher.
 \end{IEEEbiography}  \begin{IEEEbiography}{Rabie Ramadan }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{{D}aniel Urieli}{\,}(daniel.urieli@gm.com) received his Ph.D.~in artificial intelligence  (AI) from the University of Texas at Austin, where he developed AI agents that won the Power Trading Agent Competition, as well as the simulated robot soccer league in the international RoboCup competition. Daniel is a Staff Researcher at General Motors, where he has co-founded the autonomous driving research group and led research on applying AI for congestion reduction and for electric vehicle energy management.
\end{IEEEbiography}  \begin{IEEEbiography}{Xia Wang }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Yanbing Wang }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Rita Xu  }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Mengsha Yao }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Yiling You }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Gergely Zachar }{\,} (gergely.zachar@vanderbilt.edu)
is a postdoctoral researcher in the Institute for Software Integrated Systems, at Vanderbilt University.
He was part of the team for the hardware and software implementation on the I-24 MOTION project.\end{IEEEbiography}  \begin{IEEEbiography}{Yibo Zhao }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Mostafa Ameli }{\,} (mostafa.ameli@univ-eiffel.fr) is an Assistant Professor in applied mathematics, computer science, and transportation science at the Transportation Engineering and Computer Science Lab (GRETTIA), University Gustave Eiffel Paris, France. With a keen interest in the crossroads of operations research and computer science, he focuses on deploying mathematical, machine-learning, and computational tools to design smarter, more resilient transportation systems. Since 2022, he is also a Research Affiliate with the Department of Electrical Engineering and Computer Sciences at the University of California, Berkeley.  \end{IEEEbiography}  \begin{IEEEbiography}{Mirza Najamuddin Baig }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Sarah Bhaskaran }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Kenneth Butts }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Manasi Gowda }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{John Lee  }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Liam Pedersen }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Zimo Zhang }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Chang Zhou }{\,} \Dan{bio missing} \end{IEEEbiography}  \begin{IEEEbiography}{Daniel B.~Work }{\,} (dan.work@vanderbilt.edu) is a Professor of Civil and Environmental Engineering and the Institute for Software Integrated Systems, at Vanderbilt University. His interests are in transportation cyber-physical systems. \end{IEEEbiography}  \begin{IEEEbiography}{Benjamin Seibold }{\,} is a Professor of Mathematics and Physics, and the Director of the Center for Computational Mathematics and Modeling, at Temple University. His research areas, funded by NSF, DOE, DAC, USACE, USDA, and PDA, are computational mathematics (high-order methods for differential equations, CFD, molecular dynamics) and applied mathematics and modeling (traffic flow, invasive species, many-agent systems, radiative transfer). \end{IEEEbiography}  \begin{IEEEbiography}{Jonathan Sprinkle }{\,} Jonathan Sprinkle is a Professor of Computer Science at Vanderbilt University since 2021. Prior to joining Vanderbilt he was the Litton Industries John M. Leonis Distinguished Associate Professor of Electrical and Computer Engineering at the University of Arizona, and the Interim Director of the Transportation Research Institute. From 2017-2019 he served as a Program Director in Cyber-Physical Systems and Smart \& Connected Communities at the National Science Foundation in the CISE Directorate.  \end{IEEEbiography}  \begin{IEEEbiography}{Benedetto Piccoli }{\,} Benedetto Piccoli is University Professor and
the Joseph and Loretta Lopez Chair Professor
of Mathematics at Rutgers University -
Camden. He also served as Vice Chancellor for
Research.
His research interests span various areas of
applied mathematics, including control theory,
traffic flow on networks, crowd dynamics, math
finance and application to autonomous driving,
population health and bio-medical systems. He
is author of more than 300 research papers and
7 books and is the founding editor of Networks
and Heterogeneous Media.
Piccoli is the recipient of the 2009 Fubini Prize,
Plenary speaker at ICIAM 2011, and 2012
inaugural Fellow of American Mathematical
Society. \end{IEEEbiography}  \begin{IEEEbiography}{Maria Laura Delle Monache }{\,} (mldellemonache@berkeley.edu) is an Assistant Professor in the Department of Civil and Environmental Engineering at the University of California, Berkeley. Dr. Delle Monache's research lies at the intersection of transportation engineering, mathematics, and control and focuses on modeling and control of mixed autonomy large-scale traffic systems. \end{IEEEbiography}  \begin{IEEEbiography}{Alexandre M.~Bayen }{\,} Alexandre Bayen is the Associate Provost for Moffett Field Program Development at UC Berkeley, and the Liao-Cho Professor of Engineering at UC Berkeley. He is a Professor of Electrical Engineering and Computer Science and of Civil and Environmental Engineering (courtesy). He is a visiting Professor at Google. He is also a Faculty Scientist in Mechanical Engineering, at the Lawrence Berkeley National Laboratory (LBNL). From 2014 - 2021, he served as the Director of the Institute of Transportation Studies at UC Berkeley (ITS). \end{IEEEbiography}    

==> FullResults.tex <==
The experimental, observational, data collection, and data processing framework described above generated a large amount of data, capturing every single vehicle on a highway during the deployment of 100 control vehicles. %"Every Single vehicle" is an inaccrate statement in my opinion for the data used here-Sulaiman
Analogous to previous seminal traffic data sets, such as NGSIM \cite{TrafficNGSIM}, the new data are expected to inspire and enable many subsequent findings. To highlight this potential, we here present some key first findings and insights, based on an analysis of the data both with a microscopic and with a macroscopic perspective.

First, we construct macroscopically meaningful fields in time--space, most prominently a field that shows the energy (in)efficiency of traffic at large on the I-24 highway segment. This is achieved by applying Edie's method~\cite{edie1961car} on boxes of size $h_t \times h_x$, where $h_t = 10\text{s}$ and $h_x = 200\text{m}$, to the I-24 MOTION trajectories to construct the following fields:
\begin{itemize}
\item vehicle density $\rho(t,x)$, as the total vehicle time spent in each box, divided by the size of the box, $h_t\cdot h_x$;
\item flow rate $q(t,x)$, as the total distance traveled in each box, divided by  $h_t\cdot h_x$; and
\item fuel rate density $f(t,x)$, as the total fuel consumed in each box, divided by $h_t\cdot h_x$.
\end{itemize}
From these fields, other meaningful fields are obtained, such as the bulk velocity field $u(t,x) = q(t,x)/\rho(t,x)$, the bulk fuel rate $\phi(t,x) = f(t,x)/\rho(t,x)$, and the bulk fuel consumption $\psi(t,x) = f(t,x)/q(t,x)$. The latter quantity $\psi(t,x)$, measureable for instance in grams per meter, represents the fuel demand per distance traveled of all vehicles in the $h_t \times h_x$ vicinity of the position $(t,x)$. Figure~\ref{fig:TS_bulkfuel} shows $\psi(t,x)$ for two experimental days: Wednesday November 16 and Thursday November 17, 2022. Each plot is overlaid with the trajectories of all control vehicles. This represents the first time that a complete time--space diagram of the energy inefficiency of traffic, based on accurate trajectories of \emph{all} vehicles on the roadway has been provided.

\begin{figure*}
    \centering
    \includegraphics[width=.99\textwidth]{2021_New_CSM_Template/figures/benni/fig_results_per_ch_of_veh_dynamics_analysis_20221117.png}
    \caption{Relative increase of performance values (from Figure~\ref{fig:results_microscopic_behind_av_and_ahead}) of a vehicle a distance behind an AV relative to the corresponding value the same distance ahead of an AV. The plots, for 11/17/2022, indicate that in the vicinity of AVs, the behavior behind versus ahead of the AV is significantly different, and with increasing distance, that difference is waning. Most importantly for energy efficiency, the fuel consumption (mean and median) at distances up to $125\text{m}$ %while the bin center (desplayed) is at 125, the data collected for that point is up to 130m, consider using bin edge (130) instead of bin center -Sulaiman
    is 5--10\% lower behind an AV that it is ahead of an AV, indicating a small but clearly notable impact of the AVs on the total energy performance of traffic.}
    \label{fig:results_microscopic_ratios_behind_over_ahead}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=.99\textwidth]{2021_New_CSM_Template/figures/benni/fig_results_per_ch_of_veh_dynamics_analysis_20221116_fuel.png}\\[.8em]
    \includegraphics[width=.99\textwidth]{2021_New_CSM_Template/figures/benni/fig_results_per_ch_of_veh_dynamics_analysis_20221118_fuel.png}
    \caption{Increase in fuel consumption of vehicles behind an AV relative to vehicles ahead of an AV at the same distance. Displayed are the same graphs as in the bottom panel in Figure~\ref{fig:results_microscopic_ratios_behind_over_ahead}, but here for Wednesday 11/16/2022 (top) and Friday 11/18/2022 (bottom). While qualitatively exhibiting a very similar behavior as Thursday 11/17/2022, the relative savings in fuel are more notable for Friday 11/18, with mean and median yielding more than 8--15\% energy savings for distances up to $105\text{m}$%same bin edge note -Sulaiman
    .}
    \label{fig:results_microscopic_ratios_behind_over_ahead_fuel}
\end{figure*}


In the same spirit as the purely microscopic Figure~\ref{fig:TS_megacontroller}, one can, for both days shown in Figure~\ref{fig:TS_bulkfuel}, clearly see the traffic waves traveling backwards along the highway, as well as the increased fuel consumption incurred in these waves. The figure also shows the increased fuel demand in the uphill segment between $x = 5\text{km}$ and $x = 6\text{km}$, and the reduced fuel demand in the downhill segment thereafter. The AV trajectories are colored red when the automated controller was activated, and white when the vehicle was under human control. The two shown test days were quite different in terms of the engagement rates of the controllers: on 11/16, the controllers were engaged 38\% of all times, while on 11/17, the engagement rate went up to 78\%. This difference was causes by a combination of increased driver comfort with the automation, and a more reliable communication of traffic information to the vehicles on 11/17.

Given the low penetration rate of the control vehicles on the highway, it was not expected that they would completely smooth out all traffic waves---and the plots in Figure~\ref{fig:TS_bulkfuel} confirm that expectation. However, the AVs may still have had some positive contribution on the energy efficiency of the flow at large. Whether that was in fact the case, we first note that the macroscopic plots like in Figure~\ref{fig:TS_bulkfuel} allows for a targeted inspection of different regions of interest in time-space. For instance, on 11/16, there is a distinct region of high fuel inefficiency, around time 08:25:00 and location 5.0km--6.5km; and notably, this high-fuel region coincides with all AV controller being inactive. In contrast, on 11/17 such clusters of inactive AVs did not occur---and the fuel consumption map does not exhibit similarly large high-fuel regions. Another notable anecdote occurs on 11/16 in the wave that goes through $x=2.3\text{km}$ at time 07:00:00. First two active AVs notably dampen the wave; then the wave keeps on growing while four inactive AVs run through it (at $x=3\text{km}$); followed by several active AVs (around $x=4\text{km}$) notably dampening the wave again.

In addition to such targeted analysis, enabled by the macroscopic fields, we also study the I-24 MOTION trajectory data microscopically, as follows. For every data point on each vehicle trajectory, the distances (in the same lane) to (a)~the nearest AV (with active controller at that time) downstream and (b)~to the nearest AV upstream are found. Then, all the data points are binned according to their distance behind the nearest AV, where negative distances denote distances ahead of an AV. Each data point is thus counted twice, except for when no AV exists downstream/upstream. Then, for all data points in each distance bin, the distributions of key vehicle behavior or performance characteristics are considered. Figure~\ref{fig:results_microscopic_behind_av_and_ahead} shows, for Thursday 11/17, the resulting  10th, 25th, 50th (median), 75th, and 90th percentile curves, as well as the curves of the mean, for the following quantities: speed, fuel rate ($\text{g}/\text{s}$) and fuel consumption ($\text{g}/\text{m}$). For the fuel consumption, data for speeds below $0.5\text{m}/\text{s}$ are excluded from the mean, because fuel per distance is not defined for non-moving vehicles.

The results in Figure~\ref{fig:results_microscopic_behind_av_and_ahead} show a significant dip in the speed distributions' width for distances below $30\text{m}$, likely caused by the systematic bias that arises in traffic waves: such short vehicle distances tend to largely arise in traffic waves, and in those, speeds tend to be low. This means that (a)~data for distances below $30\text{m}$ may not be reliable, %reliable for what exactly? I assume it's not realiable to quantify the effect of the AV. -Sulaiman
but (b)~data above that threshold appear devoid of such bias. Finally, the graphs for both energy performance characteristics, that is fuel rate ($\text{g}/\text{s}$) and fuel consumption ($\text{g}/\text{m}$), generally have lower values behind an AV than they have ahead of an AV. Below we quantify these trends.

The previous graphs indicate that data at distances between $40\text{m}$ and $100\text{m}$ appear both reliable and most significant. Hence, in Figure~\ref{fig:results_microscopic_histograms}, we consider the distributions of key performance characteristics in this distance regime, and compare the distribution behind an AV against the distribution ahead of an AV. The plots reveal that (i)~behind an AV speed are less often close to zero than ahead of an AV, and (ii)~fuel-efficient driving occurs more frequently behind an AV (in both fuel rate and fuel consumption).

Finally, the relative increase of key performance values of vehicles a distance behind an AV versus the corresponding value the same distance ahead of an AV is considered. For the same day as above, 11/17/2022, Figure~\ref{fig:results_microscopic_ratios_behind_over_ahead} shows the resulting curves (at distances above the bias threshold) for speed, fuel rate, and fuel consumption. First, the fuel data clearly indicate the expected fact that for shorter distances, it plays a stronger role whether a vehicle is behind or ahead of an AV than it does for larger distances. Second, when considering the fuel consumption, which is the critical quantity for energy efficiency, one can see that both for mean and median, at distances up to $125\text{m}$%same bin edge comment -sulaiman
, being behind an AV results in 5--10\% lower fuel consumption relative to being ahead of an AV at the same distance. This indicates a small but clearly notable impact of the AVs on the energy performance of other vehicles in the traffic stream. As AVs with the specifically designed controllers were also deployed on 11/16 and 11/18, we display in Figure~\ref{fig:results_microscopic_ratios_behind_over_ahead_fuel} the relative fuel consumption (behind versus ahead an AV). The general trends are the same on those other two days, with equal (11/16) or even better fuel savings, yielding between 8--15\% lower energy demand on 11/18 for distances up to $105\text{m}$.%bin edge -Sulaiman

These results also reveal why the macroscopic plots in Figure~\ref{fig:TS_bulkfuel} still exhibit waves despite the presence of control vehicles: with only 100 AVs, the average distance between successive active AVs in each lane is larger than $250\text{m}$, while the AVs' notable impact wanes at less than half that distance. At the same time, these results also indicate that if one were to upscale the penetration rate of AVs with well-designed controllers, then a 10\% reduction of the overall fuel demand of traffic should be possible. 


==> sidebar_guidelines.tex <==
\begin{sidebar}{Sidebars in {\it IEEE Control Systems}}

\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}

\sdbarinitial{A} sidebar is a self-contained digression that provides additional information in support of  the main text. Sidebars are strongly encouraged since readers find these digressions useful and informative. Place sidebars throughout the document, starting each one on a new page. Every sidebar must be mentioned in the main text using the style `For details, see ``How Does Fusion Work?''' The technique for referencing sidebars in the main body of the text is as follows. The  sidebar title is created using the command

\begin{verbatim}\section[How Does Fusion Work?]{Sidebar: 
   How Does Fusion Work?} \label{sidebar-HDFW}.\end{verbatim}

The text might then include a sentence such as, `See ``\verb|\nameref{sidebar-HDFW}|'' for more details on techniques that can be used to increase the controller robustness.' You will need to add \verb|\usepackage[draft]{hyperref}| for this to work.

\sdbarfig{\includegraphics[width=19.0pc]{figures/fig1.eps}}{Note that figures in sidebars are numbered as S1, S2, and so on, to distinguish them from ones in the main text of the article.\label{sfig1}}

Figures and tables in sidebars are numbered as Figure \ref{sfig1} and Table \ref{stab1}. If the first sidebar has Figure \ref{sfig1} and Figure S2, then the first figure in the second sidebar is numbered S3. The same numbering scheme is used for equations and tables that appear in sidebars. To manually label sidebar equations in LaTeX, use \verb|tag*{\mbox{\rm{S4}}}|. Sidebar equations and figures  can be automatically numbered by using the commands listed below.

\bgroup{\fontsize{7.5pt}{12pt}\selectfont\begin{verbatim}
\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}
\end{verbatim}}\egroup

\sdbartable{Units for magnetic
properties.\label{stab1}}{\begin{tabular*}{18.5pc}{@{}|p{27pt}|p{67pt}<{\raggedright}|p{90pt}<{\raggedright}|@{}}
\hline
&  & \textbf{Conversion from} \\
&  & \textbf{Gaussian and  CGS} \\
\textbf{Symbol} & \textbf{Quantity} & \textbf{EMU to SI}$^{\mathrm{a}}$ \\
\hline
$\Phi $& 
Magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V $\cdot$ s \\
$B$& 
Magnetic flux density,   magnetic induction& 
1 G $\to  10^{-4}$ T $=$\break $10^{-4}$ Wb/m$^{2}$ \\
$H$& 
Magnetic field strength& 
1 Oe $\to  10^{-3}/(4\pi )$ A/m \\
$m$& 
Magnetic moment& 
1 erg/G $=$ 1 emu   $\to$\break $10^{-3}$ A $\cdot$ m$^{2} = 10^{-3}$ J/T \\
$M$& 
Magnetization& 
1 erg/(G $\cdot$ cm$^{3}) =$\break 1 emu/cm$^{3}$   $\to 10^{-3}$ A/m \\
\hline
\end{tabular*}}

A sidebar can cite references from the bibliography of the main text or it can have its own bibliography using the numbering style [S1], [S2]. The same scheme is used for sidebar figures and tables. See the ``Use of References in a Sidebar'' section for further details. Sidebar references can be  manually numbered as follows.

\begin{verbatim}
\begin{thebibliography}{99}
\bibitem[S7]{Kailath} T. Kailath, {\em Linear 
   Systems}, Prentice Hall, 1980.
\bibitem[S8]{Courant} R. Courant and D. Hilbert, 
   {\em Methods of Mathematical Physics}, 
   Interscience, 1953.
\end{thebibliography}
\end{verbatim}

Sidebar references can also be automatically numbered using these steps:

\begin{enumerate}

\item Place each part of the article that is to have a separate bibliography in an include file, with \verb|\bibliography| as the last line.

\item Add \verb|\usepackage{chapterbib}| in the main latex file.

\item Run latex and bibtex as usual.

\item Comment out the \verb|\usepackage{chapterbib}| and all \verb|\bibliography| and \verb|\bibliographystyle| commands.

\item Copy the .bbl files into the main latex file.

\item Run latex and comment out duplicate \verb|\bibitem| entries in the sidebar bibliographies.

\item Relabel the references in the sidebars as \verb|\bibitem[S1]{...}|.

\end{enumerate}

\section{Sidebar level heading}

Sidebars must be cited in the text. The sidebars will be placed in the   text in the order in which they are mentioned. Note that all figures and tables in the sidebars must also be cited in numerical order in the sidebar. 

\end{sidebar}

\begin{sidebar}{\continuesidebar}

\setcounter{sequation}{0}
\renewcommand{\thesequation}{S\arabic{sequation}}
\setcounter{stable}{0}
\renewcommand{\thestable}{S\arabic{stable}}
\setcounter{sfigure}{0}
\renewcommand{\thesfigure}{S\arabic{sfigure}}

\subsection{Sidebar Sub Level Head}

Equation numbers in a sidebar start with S, the same as figures and tables. Equation numbers must be sequential. Equation numbering can be continued from one sidebar to another. For example, if the last equation number in this sidebar is (S10), the first numbered equation in the next sidebar would be (S11).

\subsection{Use of References in a Sidebar}

Here is some random text showing how references are handled for a sidebar. Reference \cite{SAA1} gives one random reference. A basic equation is
\begin{sequation}
f = ma,\label{seq1}
\end{sequation}
and the impact of \eqref{seq1} is highlighted in Figure \ref{sfig1}. Reference \cite{SAA2} gives another random reference, but \cite{AA1} and \cite{BB1} are references in the main body of the text that can be cited in the sidebar.

\begin{thebibliography}{S1}
\bibitem[S1]{SAA1}
T. E. Passenbrunner, M. Sassano, M. Hirsch, and L. del Re,
``Identification and inverse torque control of hydrodynamic
dynamometers,'' \textit{IEEE Trans. Control Syst. Technol.}, vol. 22, no. 2,
pp. 607--617, Mar. 
2014. doi: 10.1109/TCST.2013.2262531.

\bibitem[S2]{SAA2}
M. Hirsch and T. E. Passenbrunner, ``Extension of static non-linear
DOE identification algorithms to dynamic systems,'' in \textit{Computer
Aided Systems Theory}, R. Moreno-D\'{i}az, F. Pichler, A.
Quesada-Arencibia, Eds. Berlin: Springer-Verlag, 2011, pp. 33--40.

\end{thebibliography}
\end{sidebar}
